MS-ASL: A Large-Scale Data Set and Benchmark for Understanding American Sign Language

Sign language recognition is a challenging and often underestimated problem comprising multi-modal articulators (handshape, orientation, movement, upper body and face) that integrate asynchronously on multiple streams. Learning powerful statistical models in such a scenario requires much data, particularly to apply recent advances of the field. However, labeled data is a scarce resource for sign language due to the enormous cost of transcribing these unwritten languages. We propose the first real-life large-scale sign language data set comprising over 25,000 annotated videos, which we thoroughly evaluate with state-of-the-art methods from sign and related action recognition. Unlike the current state-of-the-art, the data set allows to investigate the generalization to unseen individuals (signer-independent test) in a realistic setting with over 200 signers. Previous work mostly deals with limited vocabulary tasks, while here, we cover a large class count of 1000 signs in challenging and unconstrained real-life recording conditions. We further propose I3D, known from video classifications, as a powerful and suitable architecture for sign language recognition, outperforming the current state-of-the-art by a large margin. The data set is publicly available to the community.

==> acronyms.tex <==
% Example:
%
% \newglossaryentry{MANET}{
%         type=\acronymtype, 
%         name={MANET},
%         description={Mobile Ad-hoc Network}, 
%         text={Mobile Ad-hoc Network}, 
%         first={Mobile Ad-hoc Network (MANET)}, 
%         plural={MANETs}, 
%         firstplural={Mobile Ad-hoc Networks (MANETs)}
% }














\newacronym{2dhmm}{2DHMM}{two-dimensional \protect\gls{hmm}}
\newacronym{aam}{AAM}{active appearance model}
\newacronym{AAM}{AAM}{active appearance model}
\newacronym{am}{AM}{acoustic model}
\newacronym{ann}{ANN}{artificial neural network}
\newacronym{ap}{AP}{average precision}
\newacronym{ar}{AR}{action recognition}
\newacronym{asl}{ASL}{American sign language}
\newacronym{ASL}{ASL}{American sign language}
\newacronym{asllrp}{ASLLRP}{American Sign Language Linguistic Research Project}
\newacronym{aslr}{ASLR}{automatic sign language recognition}
\newacronym{ASLR}{ASLR}{Automatic sign language recognition}
\newacronym{asr}{ASR}{automatic speech recognition}
\newacronym{ASR}{ASR}{automatic speech recognition}
\newacronym{AU}{AU}{action unit}
\newacronym{au}{AU}{action unit}
\newacronym{auc}{AUC}{area under curve}
\newacronym{auslan}{Auslan}{Australian sign language}
\newacronym{avsr}{AVSR}{audio-visual speech recognition}
\newacronym{bcc}{BCC}{binary connected components analysis}
\newacronym{bfgs}{BFGS}{Broyden-Fletcher-Goldfarb-Shanno}
\newacronym{bhmm}{BHMM}{Bernoulli \protect\gls{hmm}}
\newacronym{bic}{BIC}{Bayesian information criterion}
\newacronym{BLSTM}{BLSTM}{bi-directional long short term memory}
\newacronym{blstm}{BLSTM}{bi-directional long short term memory}
\newacronym{bovw}{BOVW}{bag of visual words}
\newacronym{bow}{BOW}{bag of words}
\newacronym{bsl}{BSL}{British sign language}
\newacronym{BSL}{BSL}{British sign language}
\newacronym{cart}{CART}{classification and regression tree}
\newacronym{CART}{CART}{classification and regression tree}
\newacronym{cbir}{CBIR}{content-based image retrieval}
\newacronym{cc}{CC}{classifier combination}
\newacronym{cer}{CER}{character error rate}
\newacronym{cmllr}{CMLLR}{constrained maximum likelihood linear regression}
\newacronym{CNN}{CNN}{convolutional neural network}
\newacronym{cnn}{CNN}{convolutional neural network}
\newacronym{cslr}{CSLR}{continuous sign language recognition}
\newacronym{ctc}{CTC}{connectionist temporal classification}
\newacronym{CTC}{CTC}{connectionist temporal classification}
\newacronym{cv}{CV}{computer vision}
\newacronym{damp}{DAMP}{DARPA Arabic machine-print}
\newacronym{dbn}{DBN}{deep belief network}
\newacronym{DBN}{DBN}{dynamic bayesian network}
\newacronym{dc}{DC}{direct current}
\newacronym{dcs}{DCS}{disparity cost slices}
\newacronym{dct}{DCT}{discrete cosine transform}
\newacronym{DCT}{DCT}{discrete cosine transform}
\newacronym{dgs}{DGS}{German sign language}
\newacronym{DGS}{DGS}{german sign language}
\newacronym{DNN}{DNN}{deep neural network}
\newacronym{dnn}{DNN}{deep neural network}
\newacronym{dog}{DoG}{difference of Gaussians}
\newacronym{dp}{DP}{dynamic programming}
\newacronym{dpf}{GPF}{dynamic partial function}
\newacronym{dpt}{DPT}{dynamic programming tracking}
\newacronym{DSGS}{DSGS}{Swiss German sign language}
\newacronym{dtw}{DTW}{dynamic time warping}
\newacronym{ebw}{EBW}{extended Baum Welch}
\newacronym{eer}{EER}{equal error rate}
\newacronym{emd}{EMD}{earth movers distance}
\newacronym{em}{EM}{expectation maximization}
\newacronym{EM}{EM}{expectation maximization}
\newacronym{er}{ER}{error rate}
\newacronym{FACS}{FACS}{Facial Action Coding System}
\newacronym{facs}{FACS}{facial action coding system}
\newacronym{fmllr}{fMLLR}{feature space \protect\glstext{mllr}}
\newacronym{fps}{fps}{frames per second}
\newacronym{FRA}{FRA}{frame recognition accuracy}
\newacronym{fra}{FRA}{frame recognition accuracy}
\newacronym{fsa}{FSA}{finite state automaton}
\newacronym{FSW}{FSW}{Formal and Regular SignWriting}
\newacronym{gdl}{GDL}{glyph dependent length}
\newacronym{ghmm}{GHMM}{Gaussian \protect\gls{hmm}}
\newacronym{gmmhmm}{GMM-HMM}{Gaussian mixture model \protect\gls{hmm}}
\newacronym{gis}{GIS}{generalised iterative scaling}
\newacronym{gmd}{GMD}{Gaussian mixture densities}
\newacronym{gmm}{GMM}{Gaussian mixture model}
\newacronym{GMM}{GMM}{Gaussian mixture model}
\newacronym{gnu}{GNU}{GNU's not Unix}
\newacronym{gpl}{GPL}{General Public License}
\newacronym{gsl}{GSL}{German sign language}
\newacronym{gtf}{GTF}{global texture features}
\newacronym{hamnosys}{HamNoSys}{Hamburg Notation System}
\newacronym{hdm}{HDM}{histogram distortion model}
\newacronym{hltpr}{HLTPR}{Human Language Technology and Pattern Recognition}
\newacronym{hmm}{HMM}{hidden Markov model}
\newacronym{HMM}{HMM}{hidden Markov model}
\newacronym{hog}{HOG}{histogram of oriented gradients}
\newacronym{HOG}{HOG}{histogram of oriented gradients}
\newacronym{hp}{HP}{hand position}
\newacronym{hsv}{HSV}{hue-saturation-value}
\newacronym{ht}{HT}{hand trajectory}
\newacronym{htk}{HTK}{Hidden Markov Model Toolkit}
\newacronym{hv}{HV}{hand velocity}
\newacronym{hwr}{HWR}{handwriting recognition}
\newacronym{iapr}{IAPR}{International Association for Pattern  Recognition}
\newacronym{icdar}{ICDAR}{International Conference on Document Analysis and Recognition}
\newacronym{icfhr}{ICFHR}{International Conference on Frontiers in Handwriting Recognition}
\newacronym{icr}{ICR}{intelligent character recognition}
\newacronym{idf}{IDF}{inverse document frequency}
\newacronym{idm}{IDM}{image distortion model}
\newacronym{ifh}{IFH}{invariant feature histogram}
\newacronym{ILSVRC}{ILSVRC}{ImageNet Large-Scale Visual Recognition Challenge}
\newacronym{ilsvrc}{ILSVRC}{ImageNet Large-Scale Visual Recognition Challenge}
\newacronym{imerr}{IER}{image error rate}
\newacronym{ip}{IP}{interest point}
\newacronym{irma}{IRMA}{Image Retrieval in Medical Applications}
\newacronym{is}{IS}{International Sign}
\newacronym{isl}{ISL}{Irish Sign Language}
\newacronym{iwr}{IWR}{intelligent word recognition}
\newacronym{iwslt}{IWSLT}{international workshop on spoken language  translation}
\newacronym{jsd}{JSD}{Jensen-Shannon divergence}
\newacronym{klt}{KLT}{Kanade-Lukas-Tomasi}
\newacronym{knn}{KNN}{$k$ nearest neighbor}
\newacronym{l1o}{L1O}{leaving one out}
\newacronym{lbfgs}{LBFGS}{limited memory \protect\gls{bfgs}}
\newacronym{lbg}{LBG}{Linde-Buzo-Gray}
\newacronym{lbp}{LBP}{local binary pattern}
\newacronym{LBP}{LBP}{local binary pattern}
\newacronym{lbw}{LBW}{Lancaster-Oslo-Bergen, Brown and Wellington}
\newacronym{lda}{LDA}{linear discriminant analysis}
\newacronym{LDA}{LDA}{linear discriminant analysis}
\newacronym{ldc}{LDC}{Linguistic Data Consortium}
\newacronym{lf}{LF}{local feature}
\newacronym{LIS}{LIS}{Italian sign language}
\newacronym{lis}{LIS}{Italian sign language}
\newacronym{LM}{LM}{language model}
\newacronym{lm}{LM}{language model}
\newacronym{lob}{LOB}{Lancaster-Oslo-Bergen}
\newacronym{lsf}{LSF}{Langue des Signes Fran{\c}aise}
\newacronym{lstm}{LSTM}{long short term memory}
\newacronym{lvcsr}{LVCSR}{large vocabulary continuous speech recognition}
\newacronym{map}{MAP}{mean average  precision}
\newacronym{mce}{MCE}{minimum classification error}
\newacronym{mds}{MDS}{multi-dimensional scaling}
\newacronym{me}{ME}{maximum entropy}
\newacronym{mfdi}{MFDI}{mean face difference image}
\newacronym{mil}{MIL}{multiple instance learning}
\newacronym{MIL}{MIL}{multiple instance learning}
\newacronym{mir}{MIR}{Mallinkrodt Institute of Radiology}
\newacronym{mit}{MIT}{Massachusetts Institute of Technology}
\newacronym{mle}{MLE}{model length estimation}
\newacronym{mllr}{MLLR}{maximum likelihood linear regression}
\newacronym{ml}{ML}{maximum likelihood}
\newacronym{mlpghmm}{MLP-GHMM}{\protect\gls{mlp}-\protect\gls{ghmm}}
\newacronym{mlp}{MLP}{multi-layer perceptron}
\newacronym{mmac}{MMAC}{Multi-Modal Arabic Corpus}
\newacronym{mmiconf}{MMI-conf}{confidence-based \protect\gls{mmi}}
\newacronym{mmi}{MMI}{maximum mutual information}
\newacronym{mmmiconf}{M-MMI-conf}{confidence-based \protect\gls{mmmi}}
\newacronym{mmmi}{M-MMI}{margin-based \protect\gls{mmi}}
\newacronym{mmpeconf}{M-MPE-conf}{confidence-based \protect\gls{mmpe}}
\newacronym{mmpe}{M-MPE}{margin-based \protect\gls{mpe}}
\newacronym{mnist}{MNIST}{modified \protect\gls{nist}}
\newacronym{mpeconf}{MPE-conf}{confidence-based \protect\gls{mpe}}
\newacronym{mpeg}{MPEG}{Moving Picture Experts Group}
\newacronym{mpe}{MPE}{minimum phone error}
\newacronym{mser}{MSER}{maximally stable extremal regions}
\newacronym{msrc}{MSRC}{Microsoft Research Cambridge}
\newacronym{mt}{MT}{machine translation}
\newacronym{mwe}{MWE}{minimum word error}
\newacronym{NGT}{NGT}{Dutch sign language}
\newacronym{ngt}{NGT}{Nederlandse Gebaren Taal}
\newacronym{nist}{NIST}{National Institute for Standards  and Technology}
\newacronym{nn}{NN}{nearest neighbour}
\newacronym{numa}{NUMA}{non-uniform memory architecture}
\newacronym{oao}{OAO}{one against one}
\newacronym{oatr}{OATR}{one against the rest}
\newacronym{ocr}{OCR}{optical character recognition}
\newacronym{odel}{DEL}{object deletion}
\newacronym{oerr}{OER}{object error rate}
\newacronym{ohsu}{OHSU}{Oregon Health and Science University}
\newacronym{oins}{INS}{object insertion}
\newacronym{oov}{OOV}{out of vocabulary}
\newacronym{osub}{SUB}{object substitution}
\newacronym{p2dhmm}{P2DHMM}{pseudo two-dimensional \protect\gls{hmm}}
\newacronym{pascal}{PASCAL}{Pattern Analysis, Statistical Modelling and Computational Learning}
\newacronym{patdb}{PATDB}{Printed Arabic Text Database}
\newacronym{paw}{PAW}{piece of Arabic word}
\newacronym{PCA}{PCA}{principal components analysis}
\newacronym{pca}{PCA}{principal components analysis}
\newacronym{pc}{PC}{personal computer}
\newacronym{pdf}{PDF}{probablity density function}
\newacronym{PDM}{PDM}{point density model}
\newacronym{pdm}{PDM}{point density model}
\newacronym{peir}{PEIR}{Pathology Education Instructional Resources}
\newacronym{poicaam}{POICAAM}{project-out inverse-compositional \protect\gls{aam}}
\newacronym{pp}{PP}{perplexity}
\newacronym{qbve}{QBVE}{query by visual example}
\newacronym{qs}{QS}{quotient of sums}
\newacronym{rampn}{RAMP-N}{\protect\Gls{rwth} Arabic Machine-Print Newspaper}
\newacronym{rasr}{RASR}{RWTH Aachen University Speech Recognizer}
\newacronym{rast}{RAST}{recognition by adaptive subdivision of the transformation space}
\newacronym{rbf}{RBF}{radial basis function}
\newacronym{rgb}{RGB}{red green blue}
\newacronym{rimes}{RIMES}{Reconnaissance et Indexiation de donn\'ees Manuscrites et de fac simil\'ES}
\newacronym{rnn}{RNN}{recurrent neural network}
\newacronym{roc}{ROC}{receiver operating characteristic}
\newacronym{roi}{ROI}{region-of-interest}
\newacronym{rprop}{RProp}{resilient backpropagation}
\newacronym{rs}{RS}{relevance score}
\newacronym{rsv}{RSV}{retrieval status value}
\newacronym{rwth-asr}{RWTH ASR}{RWTH Aachen University Speech Recognition}
\newacronym{rwth-ocr}{RWTH OCR}{RWTH Aachen University Optical Character Recognition}
\newacronym{rwth}{RWTH}{RWTH Aachen University}
\newacronym{sat}{SAT}{speaker adaptive training}
\newacronym{see}{SEE}{signed exact English}
\newacronym{SGD}{SGD}{stochastic gradient descent}
\newacronym{sgd}{SGD}{stochastic gradient descent}
\newacronym{sift}{SIFT}{scale invariant feature transformation}
\newacronym{signspeak}{SignSpeak}{SignSpeak}
\newacronym{slt}{SLT}{sign language translation}
\newacronym{slr}{SLR}{sign language recognition}
\newacronym{SL}{SL}{sign language}
\newacronym{sl}{SL}{sign language}
\newacronym{smt}{SMT}{statistical machine translation}
\newacronym{ssd}{SSD}{sum of squared distances}
\newacronym{SSL}{SSL}{Swedish sign language}
\newacronym{ssl}{SSL}{Swedish sign language}
\newacronym{surf}{SURF}{speeded-up robust features}
\newacronym{svd}{SVD}{singular value decomposition}
\newacronym{svm}{SVM}{support vector machine}
\newacronym{sv}{SV}{support vector}
\newacronym{swv}{SWV}{supervised writing variants}
\newacronym{tcstar}{TC-STAR}{Technology and Corpora for Speech to  Speech Translation}
\newacronym{tc}{TC}{technical committee}
\newacronym{TDPs}{TDPs}{time distortion penalties}
\newacronym{tdps}{TDPs}{time distortion penalties}
\newacronym{tdp}{TDP}{time distortion penalty}
\newacronym{ter}{TER}{tracking error rate}
\newacronym{tet}{TET}{PDFlib Text Extraction Toolkit}
\newacronym{tfidf}{TF/IDF}{text frequency/inverse document frequency}
\newacronym{tf}{TF}{text frequency}
\newacronym{trap}{TRAP}{TempoRAl Pattern}
\newacronym{trec}{TReC}{Text Retrieval Conference}
\newacronym{ttr}{TTR}{types/token ratio}
\newacronym{uibk}{UIBK}{University of Innsbruck}
\newacronym{upv}{UPV}{Universidad Polit{\'e}cnica de Valencia}
\newacronym{url}{URL}{unique resource locator}
\newacronym{usps}{USPS}{US Postal Service}
\newacronym{uw}{UW}{University of Washington}
\newacronym{vjd}{VJD}{Viola \& Jones Detector}
\newacronym{vjt}{VJT}{Viola \& Jones Tracker}
\newacronym{vj}{VJ}{Viola \& Jones}
\newacronym{vm}{VM}{visual model}
\newacronym{voc}{VOC}{visual object classes challenge}
\newacronym{vsa}{VSA}{visual speaker adaptation}
\newacronym{vts}{VTS}{virtual training sample}
\newacronym{wat}{WAT}{writer adaptive training}
\newacronym{wer}{WER}{word error rate}
\newacronym{wta}{WTA}{winner-takes-all}
\newacronym{zow}{ZOW}{zero-order warping}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../thesis"
%%% TeX-PDF-mode: t
%%% ispell-local-dictionary: "english"
%%% End:

